FLAG: Flow-based 3D Avatar Generation from Sparse Observations

To represent people in mixed reality applications for collaboration and communication, we need to generate realistic and faithful avatar poses. However, the signal streams that can be applied for this task from head-mounted devices (HMDs) are typically limited to head pose and hand pose estimates. While these signals are valuable, they are an incomplete representation of the human body, making it challenging to generate a faithful full-body avatar. We address this challenge by developing a flow-based generative model of the 3D human body from sparse observations, wherein we learn not only a conditional distribution of 3D human pose, but also a probabilistic mapping from observations to the latent space from which we can generate a plausible pose along with uncertainty estimates for the joints. We show that our approach is not only a strong predictive model, but can also act as an efficient pose prior in different optimization settings where a good initial latent code plays a major role.

==> sections/dataset_details.tex <==

\begin{table}[]
    \centering
        \caption{Detailed statistics of AMASS datasets we used in this paper.}
    \label{tab:amass}
    \begin{tabular}{l c c c}
    \toprule
    Dataset & Subjects & Motions & Minutes \\
    \midrule
    CMU & 106 & 2083 & 551.56 \\
    MPI Limits & 3 & 35 & 20.82 \\
    Total Capture  & 5 & 37 & 41.10 \\
    Eyes Japan & 12 & 750 & 363.64 \\
    KIT & 55 & 4232 & 661.84\\
    BioMotionLab & 111 & 3060 & 522.69\\
    HumanEva & 3 & 28 & 8.48\\
    EKUT & 4 & 349 & 30.71\\
    ACCD & 20 & 256 & 26.76 \\
    BMLMovi & 86 & 1801 & 168.99 \\
    MPI Mosh & 19 & 77 & 16.53\\
    SFU & 7 & 44 & 15.23\\
    Transition & 1 & 110 & 15.10\\
    MPI HDM05 & 4 & 215 & 144.54\\
    \bottomrule
    \end{tabular}

\end{table}

In this paper, we use AMASS~\cite{AMASS:ICCV:2019} for training and evaluation. AMASS is one of the largest publicly available datasets of human motion (299,234 minutes of capture). It unifies different optical marker-based motion capture datasets by representing them within a common framework with consistent parameterization. AMASS comprises 20 datasets, from which We use the suggested training and test subsets. While we keep the original test set, we remove the dataset containing dance sequences from our dataset (similar to~\cite{rempe2021humor}). The train/test datasets splits we used are listed below: 

\noindent\textbf{Training datasets.}
CMU~\cite{CMUMocap}, MPI Limits~\cite{akhter2015pose}, Total Capture~\cite{trumble2017total}, Eyes Japan~\cite{eyesJapan}, KIT~\cite{mandery2015kit}, BioMotionLab~\cite{troje2002decomposing}, BMLMovi~\cite{AMASS:ICCV:2019}, EKUT~\cite{mandery2015kit}, ACCAD~\cite{ACCAD}, MPI Mosh~\cite{loper2014mosh}, SFU~\cite{ying2011sfu}, and MPI HDM05~\cite{akhter2015pose} 

\noindent\textbf{Test datasets.}
HumanEva~\cite{sigal2010humaneva},  Transition~\cite{AMASS:ICCV:2019}

In Table~\ref{tab:amass}, we provide details of each dataset in AMASS.



==> sections/implementation_details.tex <==
In this section, we provide implementation details of different components of our approach.

\paragraph{Flow-based model $f_\theta$.}
Our flow-based model, $f_\theta$ is a RealNVP~\cite{dinh2016density} with 16 transformation blocks. Each block is an affine coupling constructed with two MLPs representing the scale and translation networks. Each MLP is composed of three fully-connected layers with hidden size 512. Note that for scale network, we consider the \texttt{Tanh} non-linearity whereas for the translation network we use \texttt{ReLU}. For both networks we use no non-linearity for the last layer. In order to make the RealNVP conditional, we incorporate the conditioning signal $[x_\mathbb{H}, \beta]$ into both scale and translation networks, therefore, the output of each affine coupling layer becomes
\begin{align}
    y_{m} = & x_m \nonumber\\
    y_{\bar{m}} = & x_{\bar{m}} \odot \exp \big(s(x_m, [x_\mathbb{H}, \beta])\big) + t(x_m, [x_\mathbb{H}, \beta])
    \label{eq:affine}
\end{align}
where $s$ is the scale network, $t$ is the translation network, $m$ are the indices of the input representation that are masked, and $\bar{m}$ are the remaining indices. After each block, we swap mask and unmask indices to avoid information loss through identity mapping (as shown in the first line of Eq.~\ref{eq:affine}).
During training, intermediate supervision is applied to blocks $IS=\{2, 4, 6, 8, 10, 12, 14\}$ with negative log-likelihood weights $w=\{\frac{2}{16},\frac{4}{16},\frac{6}{16},\frac{8}{16},\frac{10}{16},\frac{12}{16},\frac{14}{16}\}$ correspondingly. During training we use $\lambda_{\text{NLL}}=1$. After the flow is trained, for generation and likelihood estimation tasks, we drop all connections used for intermediate supervision. Since intermediate supervision is only applied during training, the model requires only one flow at test time. At the cost of increasing the \emph{training} time {\small $\sim 70\%$}, intermediate supervision improves the performance considerably. 

\paragraph{Transformer model.}
Following standard practice, our input to the transformer model is first mapped to learned embedding space with an MLP, consisting of a fully-connected layer that maps the data dimension to 256, followed by a \texttt{LeakyReLU}. The transformer encoder consists of 3 encoder layers, each with an embedding size of 256, 8 attention heads, and a feed-forward network with the hidden size of 512. Before passing the embedded representation to the transformer encoder, we add positional encoding to retain the joints order. The output of the transformer encoder is then pooled down to the representation of head and hands. The auxiliary task of masked joint prediction is done by a single fully-connected layer. Mapping to the categorical latent space is done via another MLP which gets as input the pooled representation of the transformer encoder and the conditioning signal $C=[x_\mathbb{H}, \beta]$. This MLP is constructed with a fully-connected layer that gets this input and maps it to a 256 dimensional embedding space, followed by a \texttt{LeakyReLU}, followed by another fully-connected layer that outputs a $G\times M$ matrix, representing the categorical latent representation. In our experiments, we found $G=64$ and $M=128$ to be sufficiently expressive for our task. From this latent representation, we sample a discrete latent variable (one-hot vector) via Gumbel-Softmax and use it as the input to the other auxiliary task of reconstructing the full pose, which is done with another MLP with two fully-connected layers and a \texttt{LeakyReLU} non-linearity in between. Finally, to compute $\mu_\mathbb{H}$ and $\Sigma_\mathbb{H}$, we use two identical MLPs, each with two fully-connected layers and a \texttt{LeakyReLU} non-linearity in between, getting as input the softmax-normalized latent representation and the conditioning signal $C$. Note that the two auxiliary tasks of masked joint prediction and full pose reconstruction are only used during training. For the loss terms weights during training, we use $\lambda_{\text{mjp}}=1$, $\lambda_{\text{rec}}=1$ and $\lambda_{\text{lra}}=1$. For weights within  $\mathcal{L}_\textbf{lra}$, we use $\alpha_{\text{nll}}=1$, $\alpha_{\text{rec}}=0.5$, and $\alpha_{\text{reg}}=0.25$.

For joint masking, we avoid masking the full body joints except head hands from the beginning, as the model finds it hard to predict masked joints. To ease the training, we proposed curriculum masking of joints, following the body kinematic tree. In this scheme, we start by masking the lower body, then torso joints, then neck and arms. By gradual masking, the model learns to reason about the full body given observed (unmasked) joints, and as the training progresses, we make the such task harder by progressively masking more joints, until we reach the  real-world scenario where only head and hands are unmasked. 

\paragraph{Training hyper-parameters.}
To train our models, we use the Adam optimizer~\cite{kingma2014adam}, with the learning rate of $0.0001$, batch size of $1024$, for $100$ epochs. For all other baselines, we follow their official implementation or the details in the original papers.

\paragraph{Optimization.}
To perform optimization in either pose space or latent space, we use limited-memory BFGS optimizer~\cite{liu1989limited}, with the history size of 10, learning rate of 1, and Strong-Wolfe line search function~\cite{nocedal2006numerical}. We perform optimization for the maximum 50 iterations, however, we evaluate the MPJPE after 2, 5, 10, 25, and 50 iterations. Note that when optimizing in the latent space, the optimizer has a freedom to move around the base distribution and find a latent code that matches the HMD signal. However, since HMD signal only contains information about the upper body, there is no constraint on the optimizer to stop it from going astray ( into regions of low-likelihood lower body poses). To prevent the optimizer from straying into regions of the latent space that may correspond to undesirable lower body poses, we add a regularizer to implicitly guide the optimizer to search in regions of the latent space that modifies the upper body to minimize $\mathcal{C}_{data}$. This is done by adding $r=||z_{opt} - \mu_{\mathbb{H}}||$, encouraging the solver to stick to the initial lower body guess.

==> sections/supp_results.tex <==
\begin{figure*}[!ht]
    \centering
    \begin{tabular}{c}
         \includegraphics[width=\textwidth]{figure/additional_qualitative/test_010.png}\\
         \includegraphics[width=\textwidth]{figure/additional_qualitative/test_012.png}\\
         \includegraphics[width=\textwidth]{figure/additional_qualitative/test_014.png}\\
    \end{tabular}
    
    \caption{Additional qualitative results. Best seen zoomed in. Note, in each segment of results, the last row represents our approach.}
    \label{fig:q1}
\end{figure*}

\begin{figure*}[!h]
    \centering
    \begin{tabular}{c}
         \includegraphics[width=\textwidth]{figure/additional_qualitative/test_021.png}\\
         \includegraphics[width=\textwidth]{figure/additional_qualitative/test_022.png}\\
         \includegraphics[width=\textwidth]{figure/additional_qualitative/test_024.png}\\
    \end{tabular}
    
    \caption{Additional qualitative results. Best seen zoomed in. Note, in each segment of results, the last row represents our approach.}
    \label{fig:q2}
\end{figure*}

\begin{figure*}[!h]
    \centering
    \begin{tabular}{c}
         \includegraphics[width=\textwidth]{figure/additional_qualitative/test_008.png}\\
         \includegraphics[width=\textwidth]{figure/additional_qualitative/test_000.png}\\
         \includegraphics[width=\textwidth]{figure/additional_qualitative/test_004.png}\\
    \end{tabular}
    
    \caption{Additional qualitative results. Best seen zoomed in. Note, in each segment of results, the last row represents our approach.}
    \label{fig:q3}
\end{figure*}

In this section, we provide additional qualitative results of our approach, as well as for all other baselines, in Fig.~\ref{fig:q1} to Fig.~\ref{fig:q3} shown in the next three pages. Note that the examples are not hand picked.



==> sections/vae_hmd.tex <==
In our comparison to the existing approaches, we note relatively high MPJPE for VAE-HMD~\cite{dittadi2021full} on the AMASS test set, we argue this is due to imperfect utilization of the latent space resulting from the particular two-stage training used in VAE-HMD.
To further investigate the behaviour, we followed the setup in the original paper and define a random train/test splits on a small dataset (MPI-HDM05~\cite{akhter2015pose}). In this case, we observed that VAE-HMD is capable of achieving a very low full body MPJPE of 2.39, which is in line with the original paper, and this is due the fact that test poses are quite similar to the poses in the training set (as a result of random splitting of frames within sequences of a single dataset). 
